Learning Algorithms via Neural Logic Networks

We propose a novel learning paradigm for Deep Neural Networks (DNN) by using Boolean logic algebra. We first present the basic differentiable operators of a Boolean system such as conjunction, disjunction and exclusive-OR and show how these elementary operators can be combined in a simple and meaningful way to form Neural Logic Networks (NLNs). We examine the effectiveness of the proposed NLN framework in learning Boolean functions and discrete-algorithmic tasks. We demonstrate that, in contrast to the implicit learning in MLP approach, the proposed neural logic networks can learn the logical functions explicitly that can be verified and interpreted by human. In particular, we propose a new framework for learning the inductive logic programming (ILP) problems by exploiting the explicit representational power of NLN. We show the proposed neural ILP solver is capable of feats such as predicate invention and recursion and can outperform the current state of the art neural ILP solvers using a variety of benchmark tasks such as decimal addition and multiplication, and sorting on ordered list.

==> Arithmetics.tex <==
Binary arithmetic tasks are among the widely used experiments in the topic of algorithm and pattern learning via DNNs. While binary operations are quite easy to learn for small size binary numbers, learning becomes very difficult as the size increases. This problem has been tackled in two different ways. In the feed-forward approach, the models are designed such that the complete input stream of symbols is processed sequentially through multiple layers and the output of the last layer generates the stream of symbols corresponding to the desired result of the arithmetic operation all at once (e.g.,\cite{kaiser2015neural}).
% 
Alternatively, this problem can be looked at as a case of the sequence-to-sequence learning problem (\cite{graves2014neural}) where we first process the input symbols one by one using a recurrent cell (e.g., an LSTM cell) and then another recurrent cell generates the output sequence of symbols sequentially while accessing all the outputs of the first recurrent layer generated at each time stamp. Various attention  mechanisms  and memory access models have also been proposed to improve the performance of these recurrent networks \cite{luong2015effective}.
%
To evaluate our proposed logical layers in such a standard task, we first consider the  addition of two long binary numbers. We represent each digit in a one-hot vector of depth=4 to denote $\{0,1,+,space\}$ symbols, where $space$ is used for padding the sequences to have identical lengths. 
%A typical input/output pair bis shown in below
%\begin{center}
%	\begin{tabular}{|l||c|c|c|c|c|c|c|c|c|c|c|}
%		\hline 
%		input stream & 1 & 0& 1& 0 & 1 & + & 1   & 1 & &  &    \\
%		\hline
%		output stream & 1& 1& 0 & 0& 0&  & &  & &  &    \\
%		\hline
%	\end{tabular}
%\end{center} 
Among the existing models in the literature, Neural GPU model \cite{kaiser2015neural} proved to be the most successful approach in solving such problems using a feed-forward network.
% 
In \cite{kaiser2015neural}, the authors proposed a model consisted of a multi-layer feed-forward network where each layer is designed using a recurrent convolutional GRU cell \cite{cho2014properties}.This model (combined with curriculum learning) is reported to attain 100\% accuracy for the addition of up to 2000 long binary numbers. 
%
In our experiments, we were also able to achieve 100\% accuracy in binary addition of any lengths we tested (we did not test above 200 long sequences though). 
%
We trained the Neural GPU using its default set of parameters but for our model we used two layers of SXOR logic with length 100 each followed by a set of DNF-CNF layers each with a hidden layer of size 50 in our feed-forward model (as shown in Fig.~\ref{fig:arithmodelFF}). Table~\ref{tbl:binaryfeedforward} compares the speed of the convergence for the two models by displaying the number of the training samples required to reach a certain level of accuracy for $n=10$ and $n=20$ digits inputs. As Table \ref{tbl:binaryfeedforward} suggests while both models are capable of reaching 100\% accuracy, our proposed model converges much faster. Our experiments show that our model reaches 99\% accuracy for various lengths in less than 200k training samples. However, it usually requires much more training samples to reach the 100\% accuracy level.
%
\begin{table}[h]
	\caption{Size of required training samples to reach certain levels of accuracy}
	\label{tbl:binaryfeedforward}
	\centering 
	\begin{tabular} {|c||c| c|c|}
		\hline
		Model   & 75\% & 90\% & 100\%  \\		
		\hline
		Neural GPU (n=10) & 77k  & 400k & 490k    \\ \hline
		Logic CNF-DNF (n=10) & 4k  & 25k & 260k    \\ \hline
		Neural GPU (n=20) & 400k  & 448k & 830k    \\ \hline
		Logic CNF-DNF (n=20) & 8k  & 45k & 610k    \\ \hline
	\end{tabular}
\end{table}
% 
%A more challenging task, however,  is to learn this kinds of problems in a recurrent fashion such that the network produces the output stream one symbol at a time using the same recurrent cell. As we mentioned, most state of the art methods uses some fancy ways of attention modeling and memory access to learn these recurrent algorithmic tasks.  While all those approaches are also applicable in our logical learning system, we focus on a simple model of only one recurrent cell that accesses the input stream at any time stamp and generate one symbol of the output alphabet at each timestamp as depicted in figure \ref{fig:arithmodelRNN}. We use a simple vanilla logical recurrent (LVRNN) (Fig. \ref{fig:logicRNN}) as our recurrent cell and we test this model for the task of adding two long decimal numbers. \colorbox{red}{probably have to remove or reduce this part of experiment}
%
\begin{figure}[htb]
	\label{fig:arithmodel}
	\centering     %%% not \center
	\subfigure[Feed-Forward Model ]{\label{fig:arithmodelFF}\includegraphics[width=45mm]{Feedforwardmodel.pdf}}
	\hspace{1mm}
	\subfigure[Recurrent Model]{\label{fig:arithmodelRNN}\includegraphics[width=55mm]{rnnmodel.pdf}}
	\caption{Feed-Forward and recurrent models used in our experiments}
\end{figure}

==> Grammer.tex <==
%In many of the publications regarding the power of the neural network model in learning algorithms, the models are claimed to reach 100\% accuracy whenever during the training they reach perfect accuracy on validation set. However, we have realized that in many experiments, even though on average the model has reduced the error rate significantly, they rarely learn the underlying logical flow of the problem fully and completely. 
In many of the works related to the algorithm learning tasks, the models are claimed to reach 100\% accuracy whenever they attain perfect accuracy on the validation set during the training. However, we confirmed via many experiments that even though  such models reduced the error rate significantly on the average, they rarely learn the underlying logical flow of the problem fully. 
%
In other words, even after achieving the perfect accuracy, these models usually continue to fluctuate. 
%
In contrast, the proposed logical layer model is usually able to learn the underlying logical flow.
%
Here, we compare the efficiency of the LSTM recurrent cell with our proposed LVRNN recurrent cell for the problem of understanding Palindrome grammar. The language of Palindrome grammar contains all strings in the form $WcW'$ where $W$ is an arbitrary string of symbols from some alphabet, $W'$ is the reverse of the string $W$, and $c$ is a divider symbol. For example, in the binary alphabet system, $"11001c10011"$ is a legal Palindrome string but $"11000c11000"$ is not. 
%
Because the number of illegal phrases is much larger than the legal phrases, we ensure that around 5\% of the training samples for each training batch are legal phrases. We use the model depicted in Fig.~\ref{fig:arithmodelRNN} and use only the last output of the recurrent network to create a discriminator network with the help of a dense layer. We train the network for the phrases of length 41 binary symbols using an ADAM optimizer \cite{kingma2014adam} with the learning rate of .001. Fig.~\ref{fig:grammer} compares the performance of the two models, in terms of the number of mismatches per 5000 samples processed during training of each epoch, versus the epoch number.
%
Here, there is a striking similarity to the conjunctive layer performance that we studied in Section~\ref{subsec::CompareMLP} (Fig.~\ref{fig:and_gate_compare}). Once again, we observed that although the MLP based network approaches to the perfect accuracy and can produce perfect results in a few epochs, it fails to fully learn the underlying pattern and continues to fluctuate and generate a few errors. On the contrary, our proposed logical layers cell (LVRNN) converges faster and reaches the perfect accuracy level without any further fluctuations afterwards. 


==> LDPC.tex <==
To evaluate the generalization, we consider learning an iterative decoding algorithm for the LDPC codes.
LDPC codes are linear error correcting codes that are widely used due to their capacity achieving performance \cite{richardson2001design}. 
%They can achieve Shannon limit of channel capacity as the length of the code becomes sufficiently large. 
%
One popular problem in the coding research is decoding these codes over the Binary Erasure Channel (BEC), where a subset of the bits in the received codeword (from the channel output) is marked as erased due to the channel corruption.
%
For BEC, decoding of the received LDPC codeword can be performed using an iterative Message Passing (MP) algorithm by enforcing the parity checks in the parity check matrix. In the case of BEC, the decoder knows the location of the erasures, and it should retrieve the erased bit by using the structure of the parity check matrix. 
%However, the success of the iterative MP methods are quite limited in the case of short-length block codes \cite{pishro2004decoding}. 
To compare the performance of MLP vs NLN in such a discrete algorithmic task we use the deep recurrent model that was introduced in \cite{payani2018ISTC} to learn the iterative decoding  using either of the two architectures. 
%Without going into details of the constructing the recursive message passing scheme, we can describe the algorithm in as recusive formula readers and  
Let $\bH \in \{0,1\}^{r \times n}$ be the parity check matrix for a length $n$ regular LDPC code with parameters $(d_v,d_c)$, i.e., $\bH$ has $d_v$ and $d_c$ non-zero elements in each column and row, respectively. We assign vector $V_i \in \real^{dim_v}$, $i \in \{1,\dots,n\}$ to each variable node and similarly vector $C_j \in \real^{dim_c}$, $j \in \{1,\dots,r\}$ to each check node.
Further, we define functions $\boldsymbol{\mathscr{F}} : \real^{ (d_c \times dim_v)} \mapsto \real^{dim_c}$, from the variable nodes to the check nodes and $\boldsymbol{\mathscr{G}} : \real^{(d_v \times dim_c)} \mapsto \real^{dim_v}$, from the check nodes to the variable nodes. Here, $dim_v$ and $dim_c$ denote the dimensions of the representation used in variable nodes and check nodes, respectively. We choose the one-hot representations of depth $3$ for each variable node where the three bit positions are correspond to values of '0', '1', and 'e' (erasure), respectively. 
%For example, if the bit value is '0', the vector is $[1,0,0]$. 
%The dimension $dim_c$ of check-node vectors is a design parameter of the model which controls the amount of information that can be sent from each check node to variable nodes.
We formulate the recursive formula for each variable node $v_i$ at time stamp $t+1$ as
\begin{equation}
\begin{aligned}
v_i^{(t+1)} &= \boldsymbol{\mathscr{G}} \big ( \, Vec ( \mathds{C}_i^{(t+1) ) } \,\big ) \quad, \text{where}\\
\mathds{C}_i^{(t+1)} &= \{ C_j^{(t+1)} | H(j,i)=1 , \ j \in \{1,\dots,r\} \, \}
\label{eq:backward}
\end{aligned}
\end{equation}
further,
\begin{equation}
\begin{aligned}
C_j^{(t+1)} &= \boldsymbol{\mathscr{F}} \big ( \, Vec (\mathds{V}_{i,j}^{(t)} )\,\big ) \quad, \text{where}\\
\mathds{V}_{i,j}^{(t)} &= \{ V_{i'}^{(t)} | H(j,i')=1 , \ i' \in \{1,\dots,n\} \, \}
\label{eq:forward},
\end{aligned}
\end{equation}
%
where $Vec$ function concatenates all the vectors in the input set.
The loss is defined as softmax cross-entropy between the estimated values of the variable nodes and the correct codeword vector, both represented as one-hot vectors of length $n$ and depth 3.
%, i.e.
%\begin{subequations}
%\begin{align}
%\mathcal{L}^{(t)} &= -\frac{1}{n} \sum_{i=1}^{n} \sum_{b=1}^{3} x_{ib}\log( {v'}_{ib}^{(t)} ) \\
%{v'}_i &= softmax( v_i )
%\end{align}
%\end{subequations}

In a typical message  passing scheme, the forward-backward functions would be alternatively calculated multiple times until the system reaches equilibrium. However, since the complexity and processing time would not always allow for the neural model for large number of iterations specially when the code length grow larger, we limit our training to only three iterations and in the testing phase, we run our model multiple iterations using the trained weights. 

To compare the performance of MLP and NLN we design the feed-forward functions $\boldsymbol{\mathscr{F}}$ and $\boldsymbol{\mathscr{G}}$ for the first model using a 2 layers MLP architecture (LDPC-MLP) and for the second model using NLN architecture (LDPC-NLN). We use comparable number of parameters in each model (e.g. for LDPC(3,6) code of length 48 we use hidden dimension of size 200 and we set $dim_c=20$.) 
%Table \ref{tbl:LDPC} summarizes the  layers dimension and type/activation functions used in each model. 
%We tried various settings and dimensions and number of layers and picked comparable settings in terms of the number of weights used in each model (see Table. \ref{tbl:LDPC}).
In both models, we generate random codewords for a regular LDPC(3,6) code of length 48 for each training epoch and set the number of message passing iteration to 3. ($t_{max}=3$). 

For the test data, we ran the trained model for many more iterations to see how much each model has generalized and learned the iterative algorithm. 
%We use erasure probability of $\epsilon=0.2$ in training and we test the models for different erasure probabilities. 
Fig~\ref{fig:ber_iter} depicts the performance of each  model in terms of bit error probability (BER).

As one may expect, the model based on MLP coverges faster and generate lower BER for the setup used in training, i.e, $t=3$. 
%since the models were trained using the same setup and MLP is in general more flexible and can reduce the cost function more efficiently. 
However, increasing the number of iterations in test time not only does not improve the accuracy for MLP based model, it even degrades the performance for $t>3$. On the other hand, as the number of iterations increases, the performance of LDPC-NLN model improves significantly as one might expect from a message passing algorithm. 

In other words, the rigid structures of the NLN architecture while may seem limiting on the surface, it allows for learning discrete-algorithms much more efficiently and can generalize better. 
Arguably, there are tricks that can help an MLP model performs better in such tasks. For example by significantly increasing the number of training iteration and enforcing the network to produce valid outcome at the end of each iterations (e.g. by aggregating partial loss of each iteration). However, we believe that the NLN models provide a more natural way for learning discrete tasks.

Fig.~\ref{fig:ber_erasure} compares the performance of our proposed decoder based on NLN  to the state of the art belief propagation algorithm when applied to the erasure decoding of LDPC(3,6) code. Here, we used $t=10$ for our model and $t=50$ for the belief propagation decoder and as figure suggests, the accuracy of our model is higher than the belief propagation decoder while using smaller number of iterations.
\begin{figure}[tb]
	\centering     %%% not \center
	\subfloat[BER per number of iterations]{\label{fig:ber_iter}\includegraphics[width=0.22\textwidth]{LDPC_ITER.pdf}}
	\subfloat[BER per erasure probability]{\label{fig:ber_erasure}\includegraphics[width=0.23\textwidth]{ber_erasure.png}}
	\caption{LDPC decoding over Erasure Channels}
	\label{fig:LDPC}
\end{figure}
%\begin{table}[h]
%	\caption{Design parameters for functions $\boldsymbol{\mathscr{F}}$ and $\boldsymbol{\mathscr{G}}$}
%	\label{tbl:LDPC}
%	\centering 
%	\begin{tabular} {|c||c| c|c|}
%		\hline
%		Function   & Dimensions & Type/Activation  \\		
%		\hline
%		MLP : $\boldsymbol{\mathscr{F}}$ & 100,30  & relu,sigmoid\\ \hline
%		MLP : $\boldsymbol{\mathscr{G}}$ & 100,100,60  & relu,relu,sigmoid\\ \hline
%		NLN : $\boldsymbol{\mathscr{F}}$ & 100,30  & SXOR,CONJ\\ \hline
%		NLN : $\boldsymbol{\mathscr{G}}$ & 200,100,6  & SXOR,CONJ,DISJ\\ \hline
%	\end{tabular}
%    \hspace{-3mm}
%\end{table}
%We designed a neural logic decoder which enforces the parity check equations in forward (from variable nodes to parity check nodes) and backward (from parity check nodes to variable nodes) via a 3 logical layers designed for each path. For example, if the $j^th$ check node is connected to the variable nodes $V_{j->j}$, then we would have $C_j = \text{CONJ} ( \text{SXOR} ( \text{SXOR} ( V_{i->j} ) ) ) $. The backward path has a similar structure. We share these parameters across each forward and backward path (effectively there are only two sets of weights one for forward path and one for the backward path). We used 100 logical SXOR functions in each SXOR layer and represented erased bit locations with $0.5$, half way from $0$ and $1$ logic representations, and trained the network using ADAM optimizer.  Figure~\ref{fig:ldpc} shows the performance of a regular LDPC(3,6) code of length 132 using our proposed decoding method and compares with the performance of iterative MP decoding for various channel erasure probabilities. 

==> LogicLayer.tex <==
Throughout this paper, we use 1 (True) and 0 (False) representations for the two states of a binary variable. The basic Boolean functions of two Boolean variables $x$ and $y$ can be written as
\begin{subequations}
\begin{align}\label{eq:BoolAlgebra}
\bar{x} &\quad=\quad  1 - x  \qquad,\qquad  \bar{y} =  1 - y \\
x \bigwedge y &\quad=\quad   xy \\
x \bigvee y &\quad=\quad \overline{\bar{x} \bigwedge \bar{y}}   \quad=\quad 1 - ( 1 - x )( 1 - y)  
\end{align}
\end{subequations}
%where $\otimes$ denotes the exclusive OR operation. 
%
This algebraic representation of the Boolean logic allows us to manipulate the logical expressions similar to the regular arithmetic. 
%
Let $\bx \in \{0,1\}^n$ be the input vector in a typical logical layer, and the Boolean vector $\by \in \{0,1\}^m$ be the corresponding layer output. 
%
For the conjunctive layer, our goal is to learn $m$ conjunction functions over $ \{0,1\}^n$ such that each function uses an arbitrary subset of the binary variables in $\bx$, e.g., $y_0 = x_1 \bigwedge x_7 \bigwedge x_8$ and $y_1 = x_0 \bigwedge x_1 \bigwedge x_2 \bigwedge x_7$ and so on. 
%
To learn such representations, we introduce membership weights $w_i^{(j)}$ to the network where $j \in \{1,\dots,m\}$ and $i \in \{1,\dots,n\}$. We define the layer outputs as
\begin{equation}\label{eq:conj}
y_{conj}^{(j)} = \prod_{i=1}^{n} \big( 1 - \sigma ( w_i^{(j)} )(1 - x_i )\big).
\end{equation}
%
where $\sigma(.)$ is a squashing function which limited the membership weights to the range of $[0,1]$. We consider two types of the squashing functions; hard thresholding via two times application of the relu functions , i.e. $\sigma(w) = \text{relu}( 1 - \text{relu} (1 - w))$ or alternatively soft thresholding sigmoid function in the form of $\sigma(w) = sigmoid( c * w)$ where we choose constant $c > 1$ to encourage the membership weights to move faster towards either $0$ (no membership) or $1$ (full membership).
%
While both methods works, we realized the sigmoid scaling method is more stable and allows us to use higher learning rates.
%
It is easy to see how the membership weight principle in (\ref{eq:conj}) works. Whenever $w_i^{(j)}$ converges to zero, the $i^{th}$ term in the product goes to 1 and hence the effect of $x_i$ in the expression vanishes. On the other hand, the corresponding term is reduced to $x_i$ if the membership weight goes to 1. 
%
In the actual implementation\footnote{Tensorflow implementations of the algorithms in the paper is available at \url{https://github.com/xxx/xxx}}, for the speed and stability, we replaced the product with the summation of the logarithm terms, i.e. $y_{CONJ}^{(j)} = \text{exp} (\sum ^{n}  \log( \epsilon +  1 -\sigma(  w_i^{(j)}) (1 - x_i )\big))$, where $\epsilon$ is a small constant added for stability. 
%Further, when the dimension of the input vector is large, we may notice that even for values of $\sigma(w)$ close to $1$, the product term would be very close to zero which makes the learning slow. In order to fix this, we can reduce the effect of the input vector dimension by dividing the 
%
This operation is always valid since all the weights and inputs are in the range $[0,1]$. 
%
The resulting layer has the same complexity of a single layer perceptron in terms of the number of multiplication/addition. However, note that our logic layer incurs a subtle extra cost due to the application of logarithm and exponential functions to convert the multiplication to addition.
%

The disjunctive layer can be defined similarly using the membership weights. We define the disjunctive layer using the De Morgan Law as
\begin{align}\label{eq:disj}
y_{DISJ}^{(j)} = 1 - \prod_{i=1}^{n}  ( 1 - \sigma( w_i^{(j)} ) \,x_i  ).
\end{align}
%
In design of new layers, we leverage the property that any arbitrary complex Boolean function can be expressed in standard Disjunctive Normal Form (DNF) or in Conjunctive Normal Form (CNF). 
%
In DNF form, the Boolean function is expressed by the disjunction of the sub-expressions which are consisted of only conjunctions. 
%
This is correspond to applying our proposed disjunction layer on the output of a conjunction layer.
To represent a Boolean function, we cascade our proposed disjunction and conjunction layers in (\ref{eq:disj}) and (\ref{eq:conj}) to form a DNF layer ( $ \text{DNF}(\bx) = \text{DISJ}( \text{CONJ} (\bx) )$ ) or in reverse to form a CNF layer ($\text{CNF}(\bx) = \text{CONJ}( \text{DISJ} (\bx) )$)

%We combine our proposed conjunctive and disjunctive layers to form two new multilayer structures denoted as CNF and DNF layers. then combine these two multi-layers to form a new CNF-DNF layer. This new layer would result in low complexity networks in learning complex expressions. 
%
%While 
The total number of logical functions over a Boolean input vector $\bx \in \{0,1\}^n$ is very large (i.e. $2^{2^n}$). Further, %\color{red}it is known that many of those functions can be expressed via a small number of clauses using CNF or DNF forms\color{black}. However, 
 in some cases, a simple clause in one of those standard forms can lead to an exponential number of clauses when expressed in the other form~\footnote{We can always convert CNF to DNF form and vice versa using De Morgan's Law.}. For example, it is easy to verify that converting  $(x_1 \bigvee x_2 ) \bigwedge (x_3 \bigvee x_4)\bigwedge\dots\bigwedge(x_{n-1} \bigvee x_{n} )$ to DNF leads to $2^{\frac{n}{2}}$ number of clauses. As such, it seems intuitive to increase the learning capability of the model by combining the CNF and DNF layers using the disjunction operator to create a CNF+DNF layer as
\begin{align}\label{eq:DNF-CNF}
y_{\text{DNF+CNF}}(\bx) \,&=\, \text{CNF}(\bx) \bigvee \text{DNF}(\bx) \\&=\, 1 - \big(1-\text{CNF}(\bx)\big) \big( 1-\text{DNF}(\bx)\big)
\end{align}
The combined CNF+DNF layer gives the model the freedom to use each of the standard forms that is more suitable to represent a Boolean function.

==> formulation.tex <==
In the most basic form, ICA assume the multivariate observation data is generated by a linear combination of the independent components we call source, i.e. $\bx^{(i)} = \bA \bs^{(i)}$. While this problem has been studied extensively [ref] and has been solved with theoretical guaranties, for the more general form of the problem in presence of noise and especially where the sources are mixed using non-linear functions instead of linear form, there has not been much success. 
